The Search Problem in Mixture Models

We consider the task of learning the parameters of a {\em single} component of a mixture model, for the case when we are given {\em side information} about that component, we call this the "search problem" in mixture models. We would like to solve this with computational and sample complexity lower than solving the overall original problem, where one learns parameters of all components. Our main contributions are the development of a simple but general model for the notion of side information, and a corresponding simple matrix-based algorithm for solving the search problem in this general setting. We then specialize this model and algorithm to four common scenarios: Gaussian mixture models, LDA topic models, subspace clustering, and mixed linear regression. For each one of these we show that if (and only if) the side information is informative, we obtain parameter estimates with greater accuracy, and also improved computation complexity than existing moment based mixture model algorithms (e.g. tensor methods). We also illustrate several natural ways one can obtain such side information, for specific problem instances. Our experiments on real data sets (NY Times, Yelp, BSDS500) further demonstrate the practicality of our algorithms showing significant improvement in runtime and accuracy.

==> app_infinite_axv.tex <==
\section{Infinite-sample analysis of the whitening method}

We defer the actual analysis of Algorithm~\ref{alg:meta-whitening}
to the appendix, but we will motivate the algorithm and give the
basic idea of the proof by showing that if $\hat A, \hat B$,
and $\hat m$ are equal to $A, B$ and $m$ respectively then
Algorithm~\ref{alg:meta-whitening} outputs $\mu_1$ and $\alpha_1$
exactly.

\begin{lemma}
  Let $m$, $A$, and $B$ be defined by in~\eqref{eq:m}, \eqref{eq:A}, and~\eqref{eq:B},
where $\mu_1, \dots, \mu_k$ are linearly independent.
If $\inr{\mu_1}{v} > \inr{\mu_i}{v}$ for all $i \ne 1$
and we apply Algorithm~\ref{alg:meta-whitening}
to $A$, $B$, and $x$, then it returns $\mu_1$ and $\alpha_1$.
\end{lemma}

\begin{proof}
Let $V$ and $D$ be as defined in Algorithm~\ref{alg:meta-whitening}.
Since $A$ has rank $k$,
\[
\sum_{i=1}^k \alpha_i D^{-1/2} V^T \mu_i \mu_i^T V D^{-1/2} = D^{-1/2} V^T A V D^{-1/2} = I_k.
\]
Defining $u_i := \sqrt{\alpha_i} D^{-1/2} V^T \mu_i$, we have
$\sum_i u_i u_i^T = I_k$, which implies that the $u_i$
are orthonormal in $\R^k$.
Now,
\[
 D^{-1/2} V^T B V D^{-1/2}
= \sum_{i=1}^k \alpha_i D^{-1/2} V^T \mu_i \mu_i^T V D^{-1/2}
= \sum_{i=1}^k \inr{\mu_i}{v} u_i u_i^T.
\]
Since $\inr{\mu_1}{v}$ was assumed to be larger than all other $\inr{\mu_i}{v}$, it follows
that $u_1$ is the largest eigenvector of
$D^{-1/2} V^T B V D^{-1/2}$. Now, if $w = V D^{1/2} u_1$ then $w = \sqrt{\alpha_1} \mu_1$.

Now, note that since the $\mu_i$ are linearly independent, there is a unique way to write
$X = V V^T X = \sum_i \alpha_i \mu_1$ as $a w + y$, where $y$ belongs to the span on $\{\mu_2, \dots, \mu_k\}$
(which is the same as the column span of $A - \alpha \mu_1 \mu_1^T = A - w w^T$). Moreover,
the unique choice of $a$ that allows this representation must satisfy $aw = \alpha_1 \mu_1$, which implies
that $a = \sqrt{\alpha_1}$. Therefore, $w/a = \mu_1$ and $a^2 = \alpha_1$.
\end{proof}




==> app_infinite_cancellation_axv.tex <==
\section{Infinite-sample analysis of the cancellation method}
\label{sec:infinite-cancellation}

In this section, we show that Algorithm~\ref{alg:meta-cancel}
produces the exact answer when fed exact input. This analysis is
redundant (because it follows from the finite-sample analysis
in Appendix~\ref{sec:finite-cancellation}), but it is much simpler
than the finite-sample analysis and also helps to motivate the
algorithm.

Again, we will defer the actual analysis to the appendix, and instead
show that Algorithm~\ref{alg:meta-cancel} returns the exact answer
when fed exact initial data. We will do this in two lemmas:
Lemmas~\ref{lem:z_psd} and \ref{lem:coord_algo_exact_stat}.

\begin{lemma}
Let $Z = \sum_{i=1}^k \gamma_i \mu_i \mu_i^T$ where $\{\mu_1, \hdots , \mu_k\}$ are linearly independent, $\mu_i \in \mathbb{R}^d, \gamma_i \in \mathbb{R}$ and $d>k$. If $\gamma_1 < 0$ and $\gamma_i >0$ for all $i \neq 1$ then $Z$ is not positive semi-definite. \label{lem:z_psd}
\end{lemma}
\begin{proof}
  Let $\Pi$ denote the projection onto the orthogonal complement of
  $\text{span} \{\mu_2, \hdots , \mu_k\}$. Let $x = \Pi \mu_1$,
  and note that $\inr{x}{\mu_1} > 0$ but $\inr{x}{\mu_i} = 0$
  for all $i \ne 1$. Hence, $x^T Z x = \gamma_1 \inr{x}{\mu_1}^2 < 0$
  and so $Z$ is not positive semi-definite.
\end{proof}


\begin{lemma}
Let $m$, $A$, and $B$ be defined by in~\eqref{eq:m}, \eqref{eq:A}, and~\eqref{eq:B},
where $\mu_1, \dots, \mu_k$ are linearly independent.
If $\inr{\mu_1}{v} > \inr{\mu_i}{v}$ for all $i \ne 1$
and we apply Algorithm~\ref{alg:meta-cancel}
to $A$, $B$, and $x$, then it returns $\mu_1$ and $\alpha_1$.
\label{lem:coord_algo_exact_stat}
\end{lemma}

\begin{proof}
  Define $w_i = \inr{\mu_i}{v}$ and let $\gamma_i = \alpha_i(1-\lambda w_i)$,
  so that
  \[
    Z_\lambda = A - \lambda B = \sum_{i=1}^k \gamma_i \mu_i \mu_i^T.
  \]
  Now for $\lambda >
  \frac{1}{w_1},$ $\gamma_1 <0$ and for all $\lambda \leq \frac{1}{w_1},$
  $\gamma_i \geq 0$ for all $i$ since $w_1 > w_i,$ for every $i \neq 1.$
  By Lemma \ref{lem:z_psd}, $\lambda^* = \frac{1}{w_1}$ is the largest
  $\lambda$ such that $Z_\lambda$ is PSD; hence,
  \[
  Z_{\lambda^*} = \sum_{i=2}^k \alpha_i (1-\lambda^* w_i) \mu_i \mu_i^T.
  \]
  The $k-1$ singular vectors $\{v_2 , \hdots , v_k\}$
  of $Z_{\lambda^*}$ forms a basis of the subspace $\mathcal{V} =
  \text{span} \{\mu_2 , \hdots , \mu_k\}.$ Let $\mathcal{V}_{\perp}$ be the
  perpendicular space of $\mathcal{V}$, and write
  $\Pi = I - V_{2:k} V_{2:k}^T$ for the orthogonal projection
  onto $\mathcal{V}_\perp$.
  Since $\Pi \mu_i = 0$ for $i \ne 1$, we have
  $x_1 = \Pi x = \alpha \Pi \mu_1$.
  
  Now define $b_1, \dots, b_k$ by $\mu_1 = \sum_{i=1}^k b_i v_i$.
  In order to prove that the algorithm returns $\mu_1$ correctly,
  we need to show that $b_i = a_i := c_i / \|x_1\|$.
  Indeed,
  \[
    c_i := v_1^T A v_i = \sum_{j=1}^k\alpha_j v_1^T \mu_j \mu_j^T v_i =
    \alpha_1 b_1 b_i,
  \]
  since $v_1^T \mu_j = 0$ for $j \ne 1$.
  On the other hand, $\|x_1\| = \alpha \|\Pi \mu_1\| = \alpha b_1$,
  and so $b_i = a_i$, as claimed. Moreover,
  $\hat{\alpha}_1 = \frac{c_1}{a_1^2} = \alpha_1$, as claimed.
\end{proof}



==> app_infinite_whitening_axv.tex <==
\section{Infinite-sample analysis of the whitening method}
\label{sec:infinite-whitening}

In this section, we show that Algorithm~\ref{alg:meta-whitening}
produces the exact answer when fed exact input. This analysis is
redundant (because it follows from the finite-sample analysis
in Appendix~\ref{sec:finite-whitening}), but it is much simpler
than the finite-sample analysis and also helps to motivate the
algorithm.

\begin{lemma}
  Let $m$, $A$, and $B$ be defined by in~\eqref{eq:m}, \eqref{eq:A}, and~\eqref{eq:B},
where $\mu_1, \dots, \mu_k$ are linearly independent.
If $\inr{\mu_1}{v} > \inr{\mu_i}{v}$ for all $i \ne 1$
and we apply Algorithm~\ref{alg:meta-whitening}
to $A$, $B$, and $x$, then it returns $\mu_1$ and $\alpha_1$.
\end{lemma}

\begin{proof}
Let $V$ and $D$ be as defined in Algorithm~\ref{alg:meta-whitening}.
Since $A$ has rank $k$,
\[
\sum_{i=1}^k \alpha_i D^{-1/2} V^T \mu_i \mu_i^T V D^{-1/2} = D^{-1/2} V^T A V D^{-1/2} = I_k.
\]
Defining $u_i := \sqrt{\alpha_i} D^{-1/2} V^T \mu_i$, we have
$\sum_i u_i u_i^T = I_k$, which implies that the $u_i$
are orthonormal in $\R^k$.
Now,
\begin{equation*}
 D^{-1/2} V^T B V D^{-1/2}
= \sum_{i=1}^k \alpha_i D^{-1/2} V^T \mu_i \mu_i^T V D^{-1/2} = \sum_{i=1}^k \inr{\mu_i}{v} u_i u_i^T.
\end{equation*}
Since $\inr{\mu_1}{v}$ was assumed to be larger than all other $\inr{\mu_i}{v}$, it follows
that $u_1$ is the largest eigenvector of
$D^{-1/2} V^T B V D^{-1/2}$. Now, if $w = V D^{1/2} u_1$ then $w = \sqrt{\alpha_1} \mu_1$.

Now, note that since the $\mu_i$ are linearly independent, there is a unique way to write
$X = V V^T X = \sum_i \alpha_i \mu_1$ as $a w + y$, where $y$ belongs to the span on $\{\mu_2, \dots, \mu_k\}$
(which is the same as the column span of $A - \alpha \mu_1 \mu_1^T = A - w w^T$). Moreover,
the unique choice of $a$ that allows this representation must satisfy $aw = \alpha_1 \mu_1$, which implies
that $a = \sqrt{\alpha_1}$. Therefore, $w/a = \mu_1$ and $a^2 = \alpha_1$.
\end{proof}



